Learning a Generative Transition Model for Uncertainty-Aware Robotic Manipulation

Robot learning of real-world manipulation tasks remains challenging and time consuming, even though actions are often simplified by single-step manipulation primitives. In order to compensate the removed time dependency, we additionally learn an image-to-image transition model that is able to predict a next state including its uncertainty. We apply this approach to bin picking, the task of emptying a bin using grasping as well as pre-grasping manipulation as fast as possible. The transition model is trained with up to 42000 pairs of real-world images before and after a manipulation action. Our approach enables two important skills: First, for applications with flange-mounted cameras, picks per hours (PPH) can be increased by around 15% by skipping image measurements. Second, we use the model to plan action sequences ahead of time and optimize time-dependent rewards, e.g. to minimize the number of actions required to empty the bin. We evaluate both improvements with real-robot experiments and achieve over 700 PPH in the YCB Box and Blocks Test.

==> figures/gan.tex <==
% BicycleGAN Architecture
\begin{figure}
    \centering
    \vspace{1.6mm}
    
    \definecolor{bis}{RGB}{14, 58, 106}
    \definecolor{bis1}{RGB}{194, 144, 54}
    \definecolor{bisp1}{RGB}{246, 192, 77}
    \definecolor{biN}{RGB}{85, 135, 168}
    \definecolor{biQ}{RGB}{246, 192, 77}
    \definecolor{biz}{RGB}{254, 181, 22}
    \definecolor{biL}{RGB}{224, 230, 243}
    
    \begin{subfigure}[t]{\linewidth}
		\centering
		
\begin{tikzpicture}[font=\scriptsize]
    \node[] (c) {};

    \node[draw, minimum height=32, minimum width=32, fill=bis, above of=c, node distance=22, text=white] (s) {$\hat{s}_{t}$};
    \node[draw, minimum height=4, minimum width=32, fill=bis, below of=s, node distance=25, text=white] (a) {$d_{t}$};
    \node[draw, minimum height=4, minimum width=32, fill=bis, below of=a, node distance=14, text=white] (r) {$r_{t}$};
    
    \node[draw, minimum height=4, minimum width=32, fill=biQ, below of=r, node distance=18] (Q) {$Q(z | B)$};
    
    \node[draw, minimum height=4, minimum width=32, fill=biN, below of=Q, node distance=18, text=white] (N) {$\mathcal{N}(z)$};
    
    \node[draw, minimum height=4, minimum width=32, fill=biL, above of=s, node distance=26] (D) {$L_1 + D$};
    
    \node[draw, minimum height=60, minimum width=2, right of=c, node distance=32] (G1) {};
    \node[draw, minimum height=40, minimum width=2, right of=G1, node distance=8] (G2) {};
    \node[draw, minimum height=20, minimum width=2, right of=G2, node distance=8] (G3) {};
    \node[draw, minimum height=40, minimum width=2, right of=G3, node distance=8] (G4) {};
    \node[draw, minimum height=60, minimum width=2, right of=G4, node distance=8] (G5) {};
    \node[draw, minimum height=12, minimum width=12, fill=white, right of=G3, node distance=0] (G) {$G$};
    
    \node[draw, minimum height=16, minimum width=30, fill=biL, below of=G, node distance=48] (KL) {$KL$};
    
    \node[draw, minimum height=32, minimum width=32, fill=bisp1, right of=G5, node distance=32] (sp1) {$\hat{s}_{t+1}^\prime$};
    
    \node[draw, minimum height=20, minimum width=2, left of=c, node distance=32] (E3) {};
    \node[draw, minimum height=40, minimum width=2, left of=E3, node distance=8] (E2) {};
    \node[draw, minimum height=60, minimum width=2, left of=E2, node distance=8] (E1) {};
    \node[draw, minimum height=12, minimum width=12, fill=white, right of=E2, node distance=0] (E) {$E$};
    
    \node[draw, minimum height=32, minimum width=32, fill=bis1, left of=E1, node distance=32] (s1) {$\hat{s}_{t+1}$};
    
    
    \draw [->] (s1.east) -- (E1.west);
    \draw [->, rounded corners=2pt] (E3.east) -- ($(E3.east) + (0.15, 0)$) -- ($(Q.west) + (-0.15, 0)$) -- (Q.west);
    \draw [->] (G5.east) -- (sp1.west);
    
    \draw [->, densely dashed, rounded corners=2pt] ($(Q.east) + (0, -0.1)$) -- ($(Q.east) + (0.15, -0.1)$) -- ($(KL.west) + (-0.15, 0.1)$) -- ($(KL.west) + (0, 0.1)$);
    \draw [->, densely dashed, rounded corners=2pt] (N.east) -- ($(N.east) + (0.15, 0)$) -- ($(KL.west) + (-0.15, -0.1)$) -- ($(KL.west) + (0, -0.1)$);
    
    \draw [->] (s.east) |- ($(G1.west) + (0, 0.75)$);
    \draw [->] (a.east) |- ($(G1.west) + (0, -0.1)$);
    \draw [->] (r.east) |- ($(G1.west) + (0, -0.5)$);
    \draw [->, densely dashed, blue, rounded corners=2pt] ($(Q.east) + (0, 0.1)$) -- ($(Q.east) + (0.1, 0.1)$) -- ($(G1.west) + (-0.15, -0.8)$) -- ($(G1.west) + (0, -0.8)$);
    
    \draw [->, densely dashed, rounded corners=4pt] (s1.west) -- ($(s1.west) + (-0.16, 0)$) |- (D.west);
    \draw [->, densely dashed, rounded corners=4pt] (sp1.east) -- ($(sp1.east) + (0.16, 0)$) |- (D.east);
\end{tikzpicture}
		
		\caption{cVAE-GAN}
		\label{subfig:cvae-gan}
	\end{subfigure}
	
	\begin{subfigure}[t]{\linewidth}
		\centering
        \vspace{3mm}

\begin{tikzpicture}[font=\scriptsize]
    \node[] (c) {};

    \node[draw, minimum height=32, minimum width=32, fill=bisp1, above of=c, node distance=2] (sp1) {$\hat{s}_{t+1}^\prime$};
    
    \node[draw, minimum height=32, minimum width=32, fill=bis1, below of=sp1, node distance=38] (s1) {$\hat{s}_{t+1}$};
    
    \node[draw, minimum height=46, minimum width=2, right of=sp1, node distance=32] (E1) {};
    \node[draw, minimum height=34, minimum width=2, right of=E1, node distance=8] (E2) {};
    \node[draw, minimum height=20, minimum width=2, right of=E2, node distance=8] (E3) {};
    \node[draw, minimum height=12, minimum width=12, fill=white, right of=E2, node distance=0] (E) {$E$};
    
    \node[draw, minimum height=16, minimum width=24, fill=biL, below of=E, node distance=35] (D) {$D$};
    
    \node[draw, minimum height=4, minimum width=32, fill=biz, right of=E3, node distance=32] (z) {$z^\prime$};
    
    \node[draw, minimum height=4, minimum width=32, fill=biL, above of=sp1, node distance=41] (L1) {$L_1$};
    
    \node[draw, minimum height=60, minimum width=2, left of=sp1, node distance=32] (G5) {};
    \node[draw, minimum height=40, minimum width=2, left of=G5, node distance=8] (G4) {};
    \node[draw, minimum height=20, minimum width=2, left of=G4, node distance=8] (G3) {};
    \node[draw, minimum height=40, minimum width=2, left of=G3, node distance=8] (G2) {};
    \node[draw, minimum height=60, minimum width=2, left of=G2, node distance=8] (G1) {};
    \node[draw, minimum height=12, minimum width=12, fill=white, right of=G3, node distance=0] (G) {$G$};
    
    \node[draw, minimum height=32, minimum width=32, fill=bis, left of=G1, node distance=32, text=white, yshift=20] (s) {$\hat{s}_{t}$};
    \node[draw, minimum height=4, minimum width=32, fill=bis, below of=s, node distance=25, text=white] (a) {$d_{t}$};
    \node[draw, minimum height=4, minimum width=32, fill=bis, below of=a, node distance=14, text=white] (r) {$r_{t}$};
    
    \node[draw, minimum height=4, minimum width=32, fill=biN, below of=r, node distance=18, text=white] (N) {$\mathcal{N}(z)$};
    
    
    \draw [->] (G5.east) -- (sp1.west);
    \draw [->] (sp1.east) -- (E1.west);
    \draw [->] (E3.east) -- (z.west);
    
    \draw [->] (s.east) |- ($(G1.west) + (0, 0.7)$);
    \draw [->] (a.east) |- ($(G1.west) + (0, -0.15)$);
    \draw [->] (r.east) |- ($(G1.west) + (0, -0.55)$);
    \draw [->, densely dashed, blue, rounded corners=2pt] (N.east) -- ($(N.east) + (0.1, 0)$) -- ($(G1.west) + (-0.15, -0.8)$) -- ($(G1.west) + (0, -0.8)$);
    
    \draw [->, densely dashed, rounded corners=2pt] ($(sp1.east) + (0, -0.32)$) -- ($(sp1.east) + (0.1, -0.32)$) -- ($(D.west) + (-0.15, 0.1)$) -- ($(D.west) + (0, 0.1)$);
    \draw [->, densely dashed, rounded corners=2pt] (s1.east) -- ($(s1.east) + (0.1, 0)$) -- ($(D.west) + (-0.15, -0.1)$) -- ($(D.west) + (0, -0.1)$);
    
    \draw [->, densely dashed, rounded corners=4pt] (N.west) -- ($(N.west) + (-0.16, 0)$) |- (L1.west);
    \draw [->, densely dashed, rounded corners=4pt] (z.east) -- ($(z.east) + (0.16, 0)$) |- (L1.east);
\end{tikzpicture}

		\caption{cLR-GAN}
		\label{subfig:clr-gan}
	\end{subfigure}

    \caption{The extended BicycleGAN architecture with both training cycles. Given an image before $\hat{s}_{t}$ and after $\hat{s}_{t+1}$ an action of type $p_t$ with reward $r_t$, the generator $G$ predicts an image state $\hat{s}_{t+1}^\prime$. Most importantly, $G$ is also conditioned on noise $z$, enabling the generator to sample from multi-modal distributions. Architecture and image based on \cite{zhu_multimodal_2017}.}
    \label{fig:bicycle-paper}
\end{figure}

==> layers/init.tex <==
%\ProvidesPackage{init}
\usetikzlibrary{quotes,arrows.meta}
\usetikzlibrary{positioning}

\def\edgecolor{rgb:blue,4;red,1;green,4;black,3}
\newcommand{\midarrow}{\tikz \draw[-Stealth,line width =0.8mm,draw=\edgecolor] (-0.3,0) -- ++(0.3,0);}

\usepackage{Ball}
\usepackage{Box}
\usepackage{RightBandedBox}


